Reinforcement Learning in Economics and Finance

Reinforcement learning algorithms describe how an agent can learn an optimal action policy in a sequential decision process, through repeated experience. In a given environment, the agent policy provides him some running and terminal rewards. As in online learning, the agent learns sequentially. As in multi-armed bandit problems, when an agent picks an action, he can not infer ex-post the rewards induced by other action choices. In reinforcement learning, his actions have consequences: they influence not only rewards, but also future states of the world. The goal of reinforcement learning is to find an optimal policy -- a mapping from the states of the world to the set of actions, in order to maximize cumulative reward, which is a long term strategy. Exploring might be sub-optimal on a short-term horizon but could lead to optimal long-term ones. Many problems of optimal control, popular in economics for more than forty years, can be expressed in the reinforcement learning framework, and recent advances in computational science, provided in particular by deep learning algorithms, can be used by economists in order to solve complex behavioral problems. In this article, we propose a state-of-the-art of reinforcement learning techniques, and present applications in economics, game theory, operation research and finance.

==> abstract.tex <==
%\begin{abstract}
xxx

\bigskip
  \noindent {\sl JEL}: C13; C18; C46; G22; G32

\bigskip
  \noindent {\em Keywords}: xx

sequential...

%\vfill

\vfill
%\end{abstract}

==> reinforcement/policy_learning.tex <==
In order to avoid computing and comparing the expected return of different actions, an agent could learn directly a mapping from states to actions. 

\subsubsection{Policy Gradient}\label{policy}
Here, we try to infer a policy that maximizes the outcomes reward from an action on an environment. Policy learning converges faster than Value-based learning process and allows continuous action space of the agent as the policy is now a parameterized function. An infinite number of actions would be computationally too expensive to optimize.\\
This approach is based on Policy Gradient Theorem from \cite{Sutton:2018:RLI:3312046}

\subsection{Approximate Solution Methods: Actor Critic}
Actor-Critics aim to take advantage of both Value \ref{value} and Policy approaches \ref{policy}. By merging them, it can benefit of continuous and stochastic environments and faster convergence of Policy learning, and sample efficiency and steady of Value one.

==> reinforcement/temp_diff.tex <==
Temporal Differences was designed to solve general problems, where we want to have, at time $t$, a prediction $\widehat{R}_t$ of the discounted sum $R_t$ of future incomes $r_t$'s,
$$
R_t = r_{t+1}+\gamma r_{t+2}+\gamma^2 r_{t+3}+\dots=\sum_{h=0}^\infty \gamma^h r_{t+1+h}
$$
Let $x_t$ denote the information available at time $t$ for the prediction, so that $\widehat{R}_t=\widehat{R}(x_t)$, and assume that $x_t$ is derived from the states of a Markov Chain. If $\gamma=0$, $\widehat{R}_t$ is the prediction at time $t$ of $r_{t+1}$, and the error is simply $r_{t+1}-\widehat{R}(x_t)$. In that case, we can use exponential smoothing to update previous predictions using a shrinkage of the error term, as \citet{Brown56} and \citet{Holt57}, $$\widehat{R}(x_t)+\alpha\big(r_{t+1}-\widehat{R}(x_t)\big)$$
where the smoothing factor $\alpha$ is here called learning rate. Of course, the same idea can be generalized for $\gamma\in[0,1]$ by substituting $R_t$ to $r_{t+1}$, and to observe that $R_t = r_{t+1}+\gamma R_{t+1}$, and then we update
$$\widehat{R}(x_t)+\alpha\big[\underbrace{r_{t+1}+\gamma \widehat{R}(x_{r+1})-\widehat{R}(x_t)}_{=\delta_{t+1}}\big],$$
where $\delta_{t+1}$ is the temporal difference error.

This approach can be used to our initial problem, since the value function satisfies the Hamilton-Jacobi-Bellman equation (\ref{eq:V:pi:hjb}), that we can interpret as $R_t(s_t,\pi(s_t)+\gamma V^{\pi}(s_{t+1}) $ as an estimate of $V^{\pi}(s_t)$. Using some learning rate $\alpha$, we update the value function from the previous state, as in \citet{Sutton} \arthur{pas de référence "Sutton"}, using
$$
V^{\pi}(s_t) \leftarrow V^{\pi}(s_t) + \alpha \cdot\big(R(s_t,\pi(s_t))+\gamma V^{\pi}(s_{t+1})  - V^{\pi}(s_t) \big)
$$
which can also be written
$$
V^{\pi}(s_t) \leftarrow (1-\alpha)V^{\pi}(s_t) + \alpha \cdot\big(R(s_t,\pi(s_t))+\gamma V^{\pi}(s_{t+1})  \big)
$$
as in exponential smoothing model, where an exponential moving average is used. $\alpha$, the learning rate is here the weight we assign to our existing model, and $1-\alpha$ is the weight we assign to the new sampled estimate. Hence,....


\subsubsection{$TD(0)$ or Monte Carlo}

Tabular $TD(0)$

\subsubsection{$TD(\lambda)$}

\citet{Sutton88} introduced the $TD(\lambda)$ family of methods ($\lambda=0$ is for $TD(0)$ while $\lambda=1$ corresponds to Monte Carlo). Consider here a prediction with a finite horizon $h$, 
$$
\sum_{k=0}^h \gamma^k r_{t+k}+\gamma^{t+h+1} .....
$$


\subsubsection{Q-learning}
$Q$-learning was introduced in \citet{watkins_q-learning_1992}. Bellman Equation (\ref{eq:bellman:q} was
$$
Q^{\pi}(s_t,a_t)=\sum_{s'\in\mathcal{S}} \big[R(s_t,a_t,s')+\gamma Q^{\pi}(s',\pi(s')) \big] T(s_t,a_t,s')
$$
and the optimal value was satisfies
$$
Q^{\star}(s_t,a_t)=\sum_{s'\in\mathcal{S}} \big[R(s_t,a_t,s')+\gamma V^{\star}(s') \big] T(s_t,a_t,s')\text{ where }
V^{\star}(s')=\max_{a'\in\mathcal{A}}\big\lbrace Q^{\star}(s',a') \big\rbrace
$$
Thus, $Q$-learning is based on the following algorithm: starting from $Q_0(s,a)$, at step $k+1$ set
$$
Q_{k+1}(s,a)=\sum_{s'\in\mathcal{S}} \big[R(s,a,s')+\gamma \max_{a'\in\mathcal{A}}\big\lbrace Q_k(s',a') \big\rbrace \big] T(s,a,s').
$$

\

A REPRENDRE L'ALGO 


\begin{algorithm}[H]
 \KwData{Discount factor $\gamma$ and learning parameter $\alpha$}
 \KwResult{....}
 initialization $Q(s,a)\leftarrow 0$ for all $s\in\mathcal{S},a\in\mathcal{A}$\;
 \For{$s\in\mathcal{S}$}{
 \While{$s'$ is not a goal}{
 choose action $a\in\mathcal{A}$ based on $Q$\;
 perform action $a$\;
 observe new state $s'$ and receive reward $r$\;
 $\displaystyle{Q(s,a) \leftarrow Q(s,a) + \alpha\big(r+\gamma \max_{a'\in\mathcal{A}}\{Q(s',a')-Q(s,a)\}\big)}$\;
 $ s \leftarrow s'$\;
}}
 \caption{$Q$-learning, \citet{watkins_q-learning_1992}}
\end{algorithm}

\textbf{Approximate $Q$-learning ?}

